Monotone Grid Drawings of Planar Graphs

A monotone drawing of a planar graph $G$ is a planar straight-line drawing of $G$ where a monotone path exists between every pair of vertices of $G$ in some direction. Recently monotone drawings of planar graphs have been proposed as a new standard for visualizing graphs. A monotone drawing of a planar graph is a monotone grid drawing if every vertex in the drawing is drawn on a grid point. In this paper we study monotone grid drawings of planar graphs in a variable embedding setting. We show that every connected planar graph of $n$ vertices has a monotone grid drawing on a grid of size $O(n)\times O(n^2)$, and such a drawing can be found in O(n) time.

==> oldtex.tex <==


%We now consider $e'$ is a non-tree edge. 









\begin{comment}
 --------------------------------------------------------------NEW writing end -----------

\newpage



We now prove that every connected planar graph $G$ has an embedding $G_\phi$ where a good spanning tree $T$ of $G_\phi$ exists by following theorem.
\begin{theorem}
Let $G$ be a planar graph. Then $G$ has a plane embedding $G_\phi$ such that $G_\phi$ contains a good spanning tree. Furthermore, $G_\phi$ can be found in linear-time.
 \label{lemmatree}
\end{theorem}
 
 \begin{proof}
  We give a constructive proof.


Initially we take a fixed embedding  $G_\gamma$ of $G$. We do a BFS on $G_\gamma$, in intermediate steps we fix our target embedding   for the induced subgraph of $G$ by the visited vertices. While we fix embedding, we mark tree edges   by red color and non-tree edges by green color. For this we need to track all visited vertices, tree edges, non-tree edges in BFS steps by taking help of color. Moreover, some green egdes will be marked as $bottom-to-top$ or  $top-to-bottom$. 

%We shall color all vertices by red color and all edges by either red color or green color. Tree $T$ will be form by the red vertices and red edges, and all non-tree edges will be colored by green edges. 

% We color all vertices by red color and all edges either by red or green color such that after finishing the coloring we get a good spanning tree $T$ with red vertices and red edges, and all non-tree edges with green color. In the intermediate steps of coloring, sometimes we change embedding $G_\gamma$. Finally, the changed embedding becomes $G_\phi$. 


%  Let $G_\gamma$ be a fixed embedding of $G$. 
 At first we color all vertices and edges of $G_\gamma$ by black color.
%  We then color every vertex by red and  every edge either red or green color as follows.
 We first set red color to a vertex $r$  on $C_o(G_\gamma)$ and start clockwise BFS starting from $r$. % In the intermediate steps of BFS, we color each vertex by red color and put green color on some edges and some of them are marked as $bottom-to-top$ or  $top-to-bottom$. 

%colored as red and all edges of the induced graph of $W$ is colored appropriately in the
Let $W=\{w_1,w_2,\ldots,w_k\}$ be the vertices visited in the previous levels of BFS. We assume that the embedding of subgraph induced by $W$ has been fixed, and tree edges and non-tree edges are colored appropriately for the subgraph induced by $W$.  We now show that how we color vertices and each edge on the next step. Let assume that we are traversing a neighbor of the vertex $w_i$. Let $v_1,v_2,\ldots,v_l$ be the vertices where $e'=(v_j,w_i)$ $(1\le j\le l)$ either black  or green edge. For each $e'$ we do following. 
 If none of the edge $e=(v_j, w_m) (k\le m > i)$ exists, then we color $v$ and edge $(w_i,v_j)$ by red color then we proceed to the next $e'$. Otherwise, a black or green edge $e=(v_j, w_m)$, $(k\le m\le i)$ exists, then %and for each green edge $e=(v_j, w_m)$ , $k\ge m\ge 1$ with  $bottom-to-top$ or  $top-to-bottom$ marked 
we do following.

% If none of the edge $e=(v_j, w_m) (k\le m > i)$ exists, we color $v$ and edge $(w_i,v_j)$ as red color.  Otherwise,
let $r, r'_1, r'_2,\ldots, r'_p, w_i,v_j$ be the vertices lie on the path $P(r,v_j)$ with red edges and let $r, r''_1, r''_2,$ $\ldots, r''_q, w_m$ be the vertices lie on the path $P(r,w_m)$ with red edge. Let  $P(r,r_h)$ $(h<p)$ and $(h<q)$ be the common path lies on the paths $P(r,v_j)$ and $P(r,w_m)$. Then  $C=\{r'_h,r'_{h+1},\ldots,$ $ r_p, w_i,v_j, w_m, $ $r''_q, r''_{q-1}, \ldots,r''_{h-1}, r''_h\}$ must be a cycle in $G_\gamma$. Let $G'_\phi$ be the subgraph of $G_\gamma$ such that $C_o(G'_\phi)=C$. %induced by the cycle $C=\{r, r'_1, r'_2,\ldots,$ $ r_p, w_i,v_j, w_m, $ $r''_q, r''_{q-1}, \ldots, r''_1\}$ in $G_\phi$ and including all the inner vertices of $C$. If $e$ is black we color $e$ by green color and then 
We now check following steps for each edge. 

%let $W'$ $(W'\in W)$ be the set of vertices such that edge $E'=(v_j,W')$ exists, we color all edges of $E'$ as green and check following

{\bf Setp 1:} The pair $\{v_j, w_m\}$ is a separation pair in $G'_\phi$.
Let $G_0, G_1,\ldots,G_k$, $G_{k+1}=\{v_j, w_m\}$ be the $(v_j, w_m)$-split components of $G'_\phi$ such that $r_h\in G_0$. We create $G^*_\phi$ from $G_\gamma$ by changing embedding  $G_\gamma$ such that  $G_1,G_2,\ldots,G_k$ are not   inside of the cycle $C$ in $G^*_\phi$. Figure~\ref{fig:sperationpair} illustrates an example of this case. 



{\bf Setp 2:} The vertex $v_j$ or $w_m$  is a cut vertex of $G'_\phi$. Let $G_0, G_1,\ldots$, $G_k$ be the connected components produced by the cut vertex $v_j$ or $w_m$ where $(r\in G_0)$.  We create $G^*_\phi$ from $G_\phi$  by changing embedding  such that  $G_1,G_2,\ldots,G_k$ are not  inside of the cycle $C$ in $G^*_\phi$. Figure~\ref{fig:biconnectedcomp}  illustrates an example of this case. 

\begin{figure}
\centering
\includegraphics[scale=1]{fig/sperationpair}
\caption{ Illustration for step 1 (the case of separation pair.)}
\label{fig:sperationpair}
\end{figure}
 


%\bf {Case 2:}  The vertex $w_m$  is a cut vertex of $G'_\phi$. Let $G_0, G_1,\ldots,G_r$ be the biconnected components produce by the cut vertex $v_j$ such that $r\in G_0$.  We create $G^*_\phi$ from $G_\phi$ such that  $G_1,G_2,\ldots,G_r$ are not inside of the cycle $C$ in $G^*_\phi$. The Figure~\ref{fig:biconnectedcomp}(b) illustrates an example of this case. 

 
 \begin{figure}
\centering
\includegraphics[scale=1]{fig/biconnectedcomp}
\caption{ Illustration for step 2 (cut vertex case.)}
\label{fig:biconnectedcomp}
\end{figure}
  
{\bf Setp 3:}
In this step we color some extra edges as green color and marked them either  $bottom-to-top$ or $top-to-bottom$. Now we may consider the following three cases.


{\bf Case 1:} The edge $e$ is a black edge.
We color $e$ by green color. 
Let the edges $e^t_1,e^t_2,\ldots, e^t_k$ be the black edges which are incident to the vertex $v_j$ between the edges $(w_i, v_j)$ and  $(v_j,w_m)$ in anti-clockwise order started from the edge $(w_i, v_j)$ in $G'_\phi$, as shown in the Figure~\ref{fig:blackedge}. We color $e^t_i$, $i\le k$ by green color and mark each of them by $top-to-bottom$. Similarly, let the edges $e^d_1,e^d_2,\ldots,e^d_l$ be the black edges which are incident to the vertex $w_m$ between the edges $(r''_q, w_m)$ and  $(v_j,w_m)$ in clockwise order started from the edge  $(r''_q, w_m)$ in $G'_\phi$ as shown in the Figure~\ref{fig:blackedge}. We color $e^t_i$, $i\le l$ by green color and mark each of them by $bottom-to-top$. 

{\bf Case 2:} The edge $e$ is a green edge with $top-to-bottom$ marked.
Let the edges $e^t_1,e^t_2,\ldots, e^t_k$ be the black edges which are incident to the vertex $v_j$ between the edges $(w_i, v_j)$ and  $(v_j,w_m)$ in anti-clockwise order in $G'_\phi$ as shown in the Figure~\ref{fig:blackedge}. We color $e^t_i$, $i\le k$ by green color and mark each of them by $top-to-bottom$.

% Similarly, let the edges $e^d_1,e^d_2,\ldots,e^d_l$ be the black edges which are incident to the vertex $w_m$ between the edges $(r''_q, w_m)$ and  $(v_j,w_m)$ in clockwise order in $G'_\phi$ as shown in the Figure~\ref{fig:blackedge}. We color $e^t_i$, $i\le l$ as green color and mark $bottom-to-top$. 

{\bf Case 3:} The edge $e$ is a green edge with $bottom-to-top$ marked.
Let the edges $e^t_1,e^t_2,\ldots, e^t_k$ be the black edges which are incident to the vertex $v_j$ between the edges $(w_i, v_j)$ and  $(v_j,w_m)$ in clockwise order in $G'_\phi$ as shown in the Figure~\ref{fig:blackedge}. We color $e^t_i$, $i\le k$ by green color and mark each of them by $bottom-to-top$. 

%Similarly, let the edges $e^d_1,e^d_2,\ldots,e^d_l$ be the black edges which are incident to the vertex $w_m$ between the edges $(r''_q, w_m)$ and  $(v_j,w_m)$ in anti-clockwise order in $G'_\phi$ as shown in the Figure~\ref{fig:blackedge}. We color $e^t_i$, $i\le l$ as green color and mark  $top-to-bottom$. 





%Some black edges edge incident to the vertex $v_j$ in $G'_\phi$ or some black edges edge incident to the vertex $w_m$ between the edges $(r''_q, w_m)$ and  $(v_j,w_m)$ in clockwise order in $G'_\phi$ as shown in the Figure~\ref{fig:blackedge}. We color all these edges as green color. 

%and $w_m$ has some black edges in $G'_\phi$ as shown in the Figure~\ref{fig:blackedge}. % We color this edges as green. Note that the all vertices of $G''_\phi$ is traveravle 

{\bf Step 4:} We set   $G_\phi=G^*_\phi$ and proceed to next BFS step on $G_\phi$.
 \end{comment}

